Methods for Collision-Free Navigation of Multiple Mobile Robots in Unknown Cluttered Environments

Navigation and guidance of autonomous vehicles is a fundamental problem in robotics, which has attracted intensive research in recent decades. This report is mainly concerned with provable collision avoidance of multiple autonomous vehicles operating in unknown cluttered environments, using reactive decentralized navigation laws, where obstacle information is supplied by some sensor system. Recently, robust and decentralized variants of model predictive control based navigation systems have been applied to vehicle navigation problems. Properties such as provable collision avoidance under disturbance and provable convergence to a target have been shown; however these often require significant computational and communicative capabilities, and don't consider sensor constraints, making real time use somewhat difficult. There also seems to be opportunity to develop a better trade-off between tractability, optimality, and robustness. The main contributions of this work are as follows; firstly, the integration of the robust model predictive control concept with reactive navigation strategies based on local path planning, which is applied to both holonomic and unicycle vehicle models subjected to acceleration bounds and disturbance; secondly, the extension of model predictive control type methods to situations where the information about the obstacle is limited to a discrete ray-based sensor model, for which provably safe, convergent boundary following can be shown; and thirdly the development of novel constraints allowing decentralized coordination of multiple vehicles using a robust model predictive control type approach, where a single communication exchange is used per control update, vehicles are allowed to perform planning simultaneously, and coherency objectives are avoided.

==> ack.tex <==
\addcontentsline{toc}{chapter}{Acknowledgments}
\begin{center}
\textbf{\large Acknowledgments}
\end{center}

First and foremost, I would like to express my sincere gratitude and appreciation to my supervisor,
Prof. Andrey Savkin, for all the guidance and encouragement he has offered me throughout the
period of this research.
\par
I would like to also thank our coauthors,
Prof. Alexey Matveev, Dr. Matt Garrett and Prof. Jayantha Katupitiya, for their collaboration and input.
I would like to thank Chris Lu for his
assistance in running experiments; Jayen Ashar, Nonie Politi,
Mazher Choudhury and Matthew McGill for generosity in lending equipment; and
Dr. Boris Savkovic, Mitra Bahadorian, Chao Wang, Rahatir Rashid, Dr. Mark Whitty and Dr. Hameed Teimoori for their technical 
help over the course of this research.
\par
Lastly, I would like to thank the Australian Government Department of Industry, Innovation, Science,
Research and Tertiary Education for the APA scholarship which allowed me to pursue this higher 
degree. This research was also supported in part by the Australian Research Council. 



==> apdxb.tex <==
\chapter{Specifications of the Agricultural Vehicle}
\label{appdxb}


 The control inputs to the tractor are the steering control signal and
 the propulsion control signal. The tractor's propulsion system is
 driven by a hydrostatic transmission system, which allows the control
 of the speed through the control of its swash plate. The swash plate
 can be controlled through electronic means by directly applying the
 required voltage by interfacing to the built-in computer of the
 tractor. This facilitated a non-invasive means of controlling the
 vehicle speed. Two separate analog voltages, generated by the
 on-board computer (note that the built-in and on-board are two
 different computers), one for forward motion and another for reverse
 motion are used to control the forward and reverse speeds of the
 tractor. These two voltage channels correspond to the forward pedal
 and reverse pedal on the tractor. All other logic to take care of
 unacceptable scenarios such as both pedals being pressed at the same
 time or a pedal voltage exceeding its range are provided by the
 built-in computer of the tractor.



 The automation of the steering however did not have the same ease of
 interfacing. Hence it was necessary to mount an additional actuator
 on the steering system.  There was no positive coupling between the
 steered position of the wheels and the steering column angular
 position. Hence the mounting of a separate steering sensor was
 necessary. A non-linear relationship exists between the steering
 sensor position and the actual steered angle of the front wheels. A
 standard well tuned PI controller was implemented to control the
 steering. The desired steering is specified as the desired steering
 sensor position. Such a command can easily be generated to correspond
 a desired steered angle through a simple table look-up. The steering
 control system operates very well with a speed of response an order
 higher than the speed of response of the tractor motion.



 Within limits (as determined by the manually controlled gear
 position), the speed of the tractor can be automatically
 controlled. The speed is obtained by averaging the rate of change of
 the encoder counts of the left and right hand rear wheel
 encoders. The rear wheels have an external diameter of 0.9 m. and the
 encoders generate 40000 counts per revolution. The on-board
 computer's time stamp is used to calculate the actual speed in m/s.



 \clearpage \section{Safety Subsystem}



 The safety subsystem is centered around the built-in computer's halt
 mode that is wired to the seat switch. A simple re-triggerable one
 shot timer circuit mimics the seat switch signal, also known as the
 watch-dog signal, and when active selects the propulsion signals
 generated by the on-board computer instead of those generated by the
 pedals. The re-triggering of the timer must take place every 128
 ms. or less, or else the watchdog signal will become inactive thereby
 switching all propulsion signals to the manual pedals. This requires
 the pedals to be pressed afresh to effect motion. If a pedal is not
 pressed or a driver is not present the tractor will be halted.



 The control software is written in such a manner that if any of the
 critical software modules fail then the watchdog will be disabled. In
 addition an operator at the remote console may also choose to disable
 the watchdog signal.



 \clearpage \section{Sensors}



 The tractor is equipped with a rich set of sensors. To measure its
 global position and orientation two GPS systems, both with 2 cm. RTK
 accuracy are
 available. %Inertial data are provided by a high quality IMU. The tractor also has a tilt sensor that can provide the roll and pitch angles.
 Other sensors include an encoder each for the two rear wheels and a
 steering position sensor sensing the displacement of the steering
 system's power cylinder. For communication between individual
 on-board components and the remote station outside the tractor, an
 Ethernet network is established and connected to an access point with
 a high gain antenna capable of 300m line-of-sight Wi-Fi
 communication.



 \clearpage \section{Software}



 \begin{figure}
   \centering
   \includegraphics[width=4in]{pathfollow/SoftwareArchitecture.pdf}
   \caption{Software architecture.}\label{pf:fig:software}
 \end{figure}



 A complete suite of software is put in place to take care of a
 variety of tasks. In addition to the on-board software modules, an
 additional module must run on a remote client. The data communication
 between the external client and the tractor's on-board computer takes
 place via the earlier mentioned Wi-Fi network. The remote module
 predominantly control the watchdog signal in addition to the mode
 selection and remote control.

 The software modules are shown in Fig.~\ref{pf:fig:software}. Each
 circle represents a software module. Each link shows the data flow
 and the cylinders represent disk storage. The mode of operation of
 the tractor is chosen by the remote module through buttons on a
 joystick attached to the remote computer. The tractor can operate in
 one of three modes, (i) Path generation, (ii) Remote control and
 (iii) Autonomous control. Depending on the mode of operation various
 different software modules move onto the critical path. Based on the
 mode chosen the \texttt{ExecChk} module sequentially executes the
 required modules and monitors the live execution of all required
 modules adhering to the stipulated precedence. If any of the critical
 modules fail, the \texttt{ExecChk} module will initiate a
 shutdown. If the \texttt{ExecChk} itself fails, it will be detected
 by all other modules. In that situation, the \texttt{TractorControl}
 module will disable the watchdog signal. As an additional safety
 measure, the human operator stands guard of the watchdog signal at
 the remote station.



 The \texttt{PathGen} module can generate a path of a predefined shape
 to align with the tractor's current position and
 orientation. Obviously, for this to function the GPS readings must be
 available hence the GPS module must run before \texttt{PathGen} can
 be run. The \texttt{SharedMem} module facilitates data exchange
 between modules. The \texttt{Server} module maintain contact with the
 remote module and receives the mode select, watchdog signal and
 remote control commands. \texttt{Sensing} module acquires GPS and
 inertial data. Two separate sub-modules, one for GPS and one for the
 IMU are used within it due to their different data rates. The
 \texttt{PathTrack} module executes high level control algorithms. The
 \texttt{TractorControl} module carries out the low level control of
 the steering and propulsion while recording all low level sensor
 data.

==> chap1.tex <==
\chapter{Introduction}
\label{chap:intro}

\section{Overview}

\label{sec:intro}

Navigation of autonomous vehicles is an important, classic research area in robotics, and many
approaches are well documented in the literature. However there are many aspects which remain an
increasingly active area of research. A review of recently proposed navigation methods
 applicable to collision avoidance is provided in Chapt.~\ref{chap:lit}.

Both single and coordinated groups of autonomous vehicles have many applications, such as industrial, office, 
and agricultural automation; search and rescue; and surveillance and inspection. All these problems
contain some similar elements, and collision avoidance in some form is almost universally needed.
Examples of compilations of potential applications may be readily found, see e.g. \cite{USDoD2005book1,
Shoenwald2000journ7}.

In contrast to initial approaches to vehicle navigation problems, the focus in the literature has
shifted to navigation laws which are capable of rigorous collision avoidance, such that
for some set of assumptions, it can be proven collisions will
  never occur. Overall, navigation systems with more general assumptions would be considered superior.
   Some examples of common assumptions are listed as follows:
  
  \begin{itemize}
    \item Vehicle models vary in complexity from velocity controlled linear models to realistic
    car-like models (see Sec.~\ref{sec:cluttered}). For example, collision avoidance for velocity
    controlled models is simpler since the vehicles can halt instantly if required; however this is physically
    unrealistic. This means a more complex model which better characterizes actual vehicles is desirable for use
    during analysis.
    \item Different levels of knowledge about the obstacles and other vehicles are required
     by different navigation strategies. This ranges from abstracted obstacle set information to allowance for the
     actual nature of realistic noisy sensor data obtained from range-finding sensors. In addition
     to the realism of the sensor model, the sensing requirements significantly varies
     between approaches -- in some vehicle implementations less powerful sensors are installed, 
     which would only provide limited 
     information to the navigation system (such as the minimum distance to the obstacle).
     \item Different assumptions about the shape of static obstacles have been proposed. To ensure
     correct behavior when operating near an obstacle when only limited information is available, it is
     often unavoidably necessary to presume smoothness properties relating to the obstacle boundary. However, approaches which have
     more flexible assumptions about obstacles would likely be more widely applicable to real world
     scenarios.
    \item Uncertainty is always present in real robotic systems, and proving a behavior occurs
    under an exact vehicle model does not always imply the same behavior will be exhibited when the system is
    implemented.
    To better reflect this, assumptions can be made describing bounded disturbance from the
  nominal model, bounded sensor errors, and the presence of communication errors.
 A review of the types of uncertainty present in vehicle systems is available 
 \cite{Dadkhah2012journ2}.
 
 
 \end{itemize}
 
While being able prove collision avoidance under broad circumstances is of utmost importance,
examples of other navigation law features which determine their effectiveness are listed as follows:
 
 \begin{itemize}
    \item Navigation laws which provably achieve the vehicle's goals are highly desirable.
  When possible, this can be generally shown by providing an upper bound on the time in which the
  vehicle will complete a finite task, however conservative this may be. However, proving goal
  satisfaction is possibly less critical than collision avoidance, so long as it can be experimentally
  demonstrated non-convergence is virtually non-existent.
  \item  In many applications, the computational ability of the vehicle is limited, and approaches
  with lower computational cost are favored. However, with ever increasing computer power, this concern
  is mainly focused towards small, fast vehicles such as miniature UAV's (for which the fast update rates required
  are not congruent with the limited computational faculties available).
  \item  Many navigation laws are constructed in continuous time. Virtually all digital control systems
  are updated in discrete time, thus navigation laws constructed in discrete time are more suitable
  for direct implementation.
  \end{itemize}

The key distinction between different approaches is the amount of information they have available
about the workspace. When full information is available about the obstacle set and a single vehicle
is present, \textit{global path planning} methods may be used to find the optimal path. When only 
local information is available, \textit{sensor based} methods are used. A subset of sensor based 
methods are \textit{reactive} methods, which may be expressed as a mapping between the sensor state and control input,
with no memory present.
\par
Recently, \textit{Model Predictive Control} (MPC) architectures have been applied to collision avoidance
problems, and this approach seems to show great potential in providing efficient
navigation, and easily extends to robust and nonlinear problems
(see Sec.~\ref{sec:mpc}). They have many favorable properties compared to the commonly used
\textit{Artificial Potential Field} (APF) methods and \textit{Velocity Obstacle} based methods, which could be generally more 
conservative when extended to higher order vehicle models. MPC continues to be developed 
and demonstrate many desirable properties for sensor based
navigation, including avoidance of moving
obstacles (see Sec.~\ref{sec:moving}), and coordination of multiple vehicles (see Sec.~\ref{sec:multiple}). Additionally,
 the use of MPC for sensor based boundary following problems has been proposed in this thesis
(see Chapt.~\ref{chap:convsingle}).


\section{Chapter Outline}


The problem statements and main contributions of each chapter are listed as follows:

 \begin{itemize}
 \item Chapt.~\ref{chap:lit} is based on \cite{hoy2013review}, and presents a review of the literature 
 relating to collision avoidance of static obstacles, moving
 obstacles, and other cooperating vehicles.
 
\item Chapt.~\ref{chap:singlevehicle} is based on \cite{Hoy2012journ5} and \cite{Hoy2012journ2}, and is concerned with the navigation of a single vehicle described by either holonomic or unicycle vehicle models with
bounded acceleration and disturbance. Collision avoidance is able to be proven, however convergence to the target is not analytically addressed (since assumptions regarding sensor data are not particularly realistic). The contributions of this chapter are the integration of the robust MPC concept
with reactive navigation strategies based on local path planning, applied to both holonomic and unicycle vehicle models with bounded acceleration and disturbance

\item Chapt.~\ref{chap:convsingle} is based on \cite{Hoy2011conf7}, and is concerned with navigation in unknown
environments where the information about the obstacle is limited to a discrete ray-based sensor
model. Collision avoidance, complete transversal of the obstacle and finite completion
time are able to be proven, however the vehicle model is assumed to be free from disturbance. To solve this problem, the MPC method from Chapt.~\ref{chap:singlevehicle} is extended to only consider the more limited obstacle information when performing the planning process.

\item Chapt.~\ref{chap:multiple} is based on \cite{Hoy2012journ2}, and is concerned with the navigation of multiple cooperating vehicles which are only allowed a limited number of communication exchanges per control update. Again, collision avoidance is able to be proven. To achieve this, a novel constraint is developed allowing decentralized robust coordination of multiple vehicles.  Unlike other approaches in this area, explicit
ordering of the vehicles is not required, each vehicle can plan trajectories simultaneously,
and no explicit coherency objectives are required.

\item Chapt.~\ref{chap:dead} is based on \cite{hoy2012dead}, and is concerned with preventing deadlocks between pairs of robots in cluttered environments. To achieve this, a simple yet original
method of resolving deadlocks between pairs of vehicles is proposed. The proposed method has the advantage of not requiring centralized computation or discrete abstraction of the state space.
\end{itemize}

In Chapts.~\ref{chap:singlevehicle} to \ref{chap:dead}, simulations and real 
world testing confirm the viability of the proposed methods. It should be emphasized they are all 
related since they all use the same basic planning and collision avoidance procedure proposed in 
Chapt.~\ref{chap:singlevehicle}.
\par
In Chapts.~\ref{chapt:rbf} to \ref{chapt:tcp}, the contribution of the author was the simulations 
and testing performed to validate some other varieties of navigation 
systems. In each of these chapters, some of the introductory
discussion, and all mathematical analysis, was contributed
by coauthors to the associated manuscript; however some details are included to assist 
understanding of the presented results. Each of these chapters are relatively independent (they solve quite distinct problems),
and some have introductions independent of Chapt.~\ref{chap:lit}.

\begin{itemize}
\item Chapt.~\ref{chapt:rbf} is based on \cite{Matveev2011conf9}, and is concerned with reactively avoiding obstacles 
and provably converging to a target using only scalar measurements about the minimum distance to 
obstacles and the angle to the target. The advantage of the proposed method is that it can be analytically shown to have the correct behavior, despite the extremely limited sensor information which was assumed to be available.

\item Chapt.~\ref{chapt:tf} is based on \cite{Savkin2012journ1}, and is again concerned with reactively avoiding obstacles 
and provably converging to a target. However in contrast to
Chapt.~\ref{chapt:rbf}, the sensor information available is the set of visible obstacle edges surrounding the vehicle. The advantage of the proposed method is that it explicitly allows for the kinematics of the vehicle, compared to equivalent control approaches proposed in the literature.

\item Chapt.~\ref{chapt:pf} is based on \cite{Matveev2010conf0}, and is concerned with outlining in more detail 
the path following approach employed in Chapt.~\ref{chap:singlevehicle}. In particular, extensive simulations and experiments
with an agricultural vehicle are documented. The advantage of the proposed method is that it explicitly allows for steering angle limits, and it has been shown to have good tracking performance in certain situations compared to other methods proposed in the literature.

\item Chapt.~\ref{chapt:fbf} is based on \cite{MSavkin2012journ1}, and is concerned with following the boundary of an obstacle using limited 
range information. In contrast to Chapt.~\ref{chap:convsingle}, only a single detection sector 
perpendicular to the vehicle is available. The advantage of the proposed method is that (compared to other equivalent methods proposed in the literature) it provides a single contiguous controller, and is analytically correct around transitions from concave to convex boundary segments.


\item Chapt.~\ref{chapt:ext} is based on \cite{MaHoSa13}, and is concerned with seeking the maximal point of a scalar environmental field. The advantage of the proposed method is that it des not require any type of derivative estimation, and it may be analytically proven to be correct in the case of time--varying environmental fields.


\item Chapt.~\ref{chapt:lst} is based on \cite{MaHoAnSa_sb}, and is concerned with
tracking level sets/isolines of an environmental field at a predefined set-point. The advantage of the proposed method is that it may be analytically proven to be correct in the case of time--varying environmental fields.


\item Chapt.~\ref{chapt:tcp} is based on \cite{matveev2013capt}, and is concerned with 
 decentralized formation control allowing a group of robots to form a 
circular `capturing' arrangement around a given target. The advantage of the proposed method is that it only requires local sensor information, allows for vehicle kinematics and does not require communication between vehicles.

\end{itemize}


Finally, Chapt.~\ref{chap:conclusions} presents a summary of the proposed methods, and outlines
several areas of possible future research. 

Appendix~\ref{apdx:helpexp} presents preliminary simulations
with a realistic helicopter model. Note the helicopter model and the text describing it was 
contributed by Dr. Matt Garratt. 

%Appendix~\ref{appdxb} describes the
% tractor vehicle used for testing in Chapt.~\ref{chapt:pf}. Note the
% tractor design and text describing it was contributed by Prof. Jayantha Katupitiya.

 

\section{Author's Publications}

As follows is a list of publications that were generated over the tenure of this thesis:

\subsection*{Journal}

\begin{enumerate}
\item Hoy, M., Matveev, A. S., Garratt, M., and Savkin, A. V. (2012) {\it Collision Free
Navigation of an Autonomous Unmanned Helicopter in Unknown Urban Environments:
Sliding Mode and MPC Approaches.} Robotica, 30(4):537--550.

\item Hoy, M., Matveev, A. S., and Savkin, A. V. (2012) {\it Collision free cooperative
navigation of multiple wheeled robots in unknown cluttered environments.}
Robotics and Autonomous Systems, 60(11):1253--1266.

\item Matveev, A. S., Hoy, M., and Savkin, A. V. (2013) {\it The Problem of Boundary Following by a Unicycle--like Robot with Rigidly Mounted Sensors.} Robotics and Autonomous Systems, 61(3):312-�327

\item Savkin, A. V. and Hoy, M. (2012) {\it Reactive and Shortest Path Navigation of a
Wheeled Mobile Robot in Cluttered Environments.} Robotica, 31(2):323--330.



\item Hoy, M. (2013) {\it A Method of Boundary Following by a Wheeled Mobile
Robot Based on Sampled Range Information.} Journal of Intelligent and Robotic Systems [accepted].

\item Zakhar'eva, A., Matveev, A. S., Hoy, M., and Savkin, A. V. (2013) {\it A strategy for target capturing with collision
avoidance for non-holonomic robots with sector
vision and range-only measurements.} Robotica [accepted].

\item Matveev, A. S. Hoy, M., Katupitiya, J., and Savkin, A. V. (2013) {\it Nonlinear Sliding Mode Control of an Unmanned
Agricultural Tractor in the Presence of Sliding
and Control Saturation.} Robotics and Autonomous Systems [accepted].

\item Matveev, A. S., Hoy, M., and Savkin, A. V. (2013) A Method for Reactive Navigation of
Nonholonomic Robots in Maze-Like Environments. Automatica [accepted].



\item Hoy, M., Matveev, A. S., and Savkin, A. V. (2013) {\it Algorithms for Collision Free 
Navigation of Mobile Robots in Complex Cluttered Environments: A Survey.} Robotica [submitted].

\item Matveev, A. S. Hoy, M., and Savkin, A. V. (2013) {\it Extremum Seeking Navigation without 
Derivative Estimation of a Mobile Robot in a Dynamic Environmental Field.} IEEE Transactions on Control System Technology [submitted].

\item Matveev, A. S., Hoy, M., Anisimov, A. M., Savkin, A. V. (2013) {\it Tracking Deforming Environmental Level Sets of Dynamic Fields without
Gradient Estimation by a Wheeled Mobile Robot.} Robotics and Autonomous Systems [submitted].

\item Matveev, A. S., Hoy, M., Savkin, A. V. (2013) {\it Kinematic Navigation of a Nonholonomic Robot for 3D Environmental
Extremum Seeking without Gradient Estimation.} Automatica [submitted].

\end{enumerate}


\subsection*{Conference}

\begin{enumerate}

\item Hoy, M. (2012) {\it Deadlock Resolution for Navigation of Wheeled Robots in
Continuous State-Space.} Proceedings of the 12th International Conference on
Automation, Robotics, Control and Vision, Guangzhou, China.

\item Matveev, A. S., Hoy, M., and Savkin, A. V. (2012) {\it Boundary Tracking by a Wheeled
Robot with Rigidly Mounted Sensors.} Proceedings of the 12th International Conference
on Automation, Robotics, Control and Vision, Guangzhou, China.

\item Zakhar'eva, A., Matveev, A. S., Hoy, M., Savkin, A. V. (2012) {\it A Strategy for
Target Capturing with Collision Avoidance for Non-Holonomic Robots with Sector
Vision and Range-Only Measurements.} Proceedings of the 2012 IEEE Multi-conference on
Systems and Control, Dubrovnik, Croatia.

\item Hoy, M. and Savkin, A. V. (2011) {\it A Method for Border Patrolling Navigation of a
Mobile Robot.} Proceedings of the 9th IEEE International Conference on Control and
Automation, Santiago, Chile.

\item Hoy, M., Matveev, A. S., and Savkin, A. V. (2011) {\it Robust Cooperative Navigation
of Multiple Wheeled Robots in Unknown Cluttered Environments.} Proceedings of the 19th
Mediterranean Conference on Control and Automation, Corfu, Greece.

\item Savkin, A. V., and Hoy, M. (2011) {\it Tangent Graph Based Navigation of a
Non-Holonomic Mobile Robot in Cluttered Environments.} Proceedings of the
19th Mediterranean Conference on Control and Automation, Corfu, Greece.

\item Matveev, A. S., Hoy, M., Savkin, A. V. (2011) {\it A Method for Reactive Navigation
of Nonholonomic Robots in the Presence of Obstacles.} Proceedings of the 18th IFAC
World Congress, Milan, Italy.

\item Hoy, M., Garrat, M., and Savkin, A. V. (2010) {\it Navigation of an Unmanned
Helicopter in Urban Environments.} Proceedings of the 11th International Conference on
Automation, Robotics, Control and Vision, Singapore.

\item Matveev, A. S., Hoy, M., and Savkin, A. V. (2010) {\it Mixed Nonlinear-Sliding Mode
Control of an Unmanned Farm Tractor in the Presence of Sliding.} Proceedings of
the 11th International Conference on Automation, Robotics, Control and Vision,
Singapore.



\item Matveev, A. S., Hoy, M., and Savkin, A. V. (2013) {\it Kinematic Navigation of a Mobile Robot for Environmental Extremum
Seeking without Derivatives Estimation.} The 10th International Conference on Control and Automation, Hangzhou, China [accepted].

\item Matveev, A. S., Hoy, M., Anisimov, A. M., Savkin, A. V. (2013) {\it Tracking of Deforming Environmental Level Sets of Dynamic Fields by a
Nonholonomic Robot without Gradient Estimation.} The 10th International Conference on Control and Automation, Hangzhou, China [accepted].



\item Matveev, A. S., Hoy, M., and Savkin, A. V. (2013) {\it Reactive Navigation of a Mobile Robot to the Moving
Extremum of a Dynamic Unknown Environmental Field without
Derivative Estimation.} The 2013 European Control Conference, Zurich, Switzerland [accepted].

\end{enumerate}





==> chap3a.tex <==
\chapter{Convergent Navigation of Single Vehicle}
\label{chap:convsingle}

This chapter will show how we may guarantee the vehicle converges to the desired target.

\clearpage \section{Pure Tracking control Law}

During a pure tracking segment, the only requirement upon trajectory is that they advance the vehicle at least a finite amount towards the vehicles target, and the best trajectory can be selected 

\clearpage \section{Switching Conditions}

$beta = 0$

no feasbile pure tracking control laws





==> chap3b.tex <==
\chapter{Avoidance of moving obstacles}
\label{chap:convsingle}

This chapter will briefly provide somewhat less profound, brief insights how the previous can extend to cases where moving obstacles are present

\clearpage \section{Known obstacles}
If the trajectory of moving obstacles is globally known, we may simply avoid the instantaneous position of the moving target. Let a time varying obstacle domain be given by $D(t)$.

\begin{Assumption}
$D(t)$ doesn't change too much.
\end{Assumption}

\clearpage \section{Pedestrian-like obstacles}

In general it would be difficult to prove collision avoidance with general moving obstacles, as even the most restrictive assumptions on their control capabilities would still lead to interception in some pathogenic scenarios.
Becasuse of this, we consider the case of 'cooperative' moving obstacles, where we place some assumption on the unknown agents behaviour.

There is naturally some tradeoff between the number of assumptions placed on a obstacles behaviour, and the similarity with completely cooperative scenarios.
Because of this, we will consider the simplest possible assumption on the robots motion.

\begin{Definition}
A \textit{pedestrian-like obstacle} will not collide with a stationary vehicle, and has holonomic dynamics with limited speed and acceleration.
\end{Definition}

==> copyright.tex <==
% UNSW PhD Thesis Copyright and Authenticity Statements
% Author: Mark Reid <mark AT threewordslong DOT com>
% Last modified: 14th August 2007
% Original markup taken from:
%   http://www.ctan.org/tex-archive/macros/latex/contrib/adfathesis/adfathesis.dtx

\newpage
\thispagestyle{empty}
\null\vfill
\begin{center}
\begin{minipage}{13cm}
\setlength{\parindent}{0cm}
\setlength{\parskip}{2ex}
{\underline{Copyright and DAI Statement}}
\par
{\rmfamily\normalsize
'I hereby grant the University of New South Wales or its agents the 
right to archive and to make available my thesis or dissertation in  
whole or part in the University libraries in all forms of media, now 
or here after known, subject to the provisions of the Copyright Act 1968. 
I retain all proprietary rights, such as patent rights. I also retain the 
right to use in future works (such as articles or books) all or part of 
this thesis or dissertation. 

I also authorize University Microfilms to use the 350 word abstract of 
my thesis in Dissertation Abstracts International (this is applicable to 
doctoral theses only).        

I have either used no substantial portions of copyright material in my 
thesis or I have obtained permission to use copyright material; where 
permission has not been granted I have applied/will apply for a 
partial restriction of the digital copy of my thesis or dissertation.'
}
\par
{\rmfamily\normalsize
Signed:\hrulefill\hspace{1cm}Date:\hrulefill
}
\par
\vspace{1.5cm}
{\underline{Authenticity Statement}}
\par
{\rmfamily\normalsize
'I certify that the Library deposit digital copy is a direct equivalent of 
the final officially approved version of my thesis. No emendation of 
content has occurred and if there are any minor variations in  
formatting, they are the result of the conversion to digital format.'
}
\par
{\rmfamily\normalsize
Signed:\hrulefill\hspace{1cm}Date:\hrulefill
}
\end{minipage}
\end{center}
\vfill\null


==> deterministicbf/thesis.tex <==
\chapter{Deteministic Reactive Collision Avoidance}

{\it \large Author's Note: The contribution of the author was the
simulation and testing sections. All other content was contributed by
 Prof. Alexey S. Matveev and Prof. Andrey
V. Savkin.}


\par
The remainder of the paper is organized as follows. In
Section~\ref{dbf:ps}, we define the problem to be considered. Section
\ref{dbf:bf} presents the sliding mode controller.
 Simulated results with a realistic helicopter model and
experimental results with a wheeled robot are described in
Sections~\ref{dbf:sim} and \ref{dbf:exp},
respectively. Section~\ref{dbf:conc} offers brief conclusions.
% A useful formula is derived in Appendix.

\section{Problem statement}
\label{dbf:ps}

We consider a helicopter traveling in the plane, which contains a
steady point target $T$ and a set of unknown, untransversable, static,
disjoint, and closed obstacles $D_i \not\ni T, i \in [1:n]$.  The
objective is to design a navigation law that drives the helicopter to
the target through the obstacle-free part of the plane $\mathbb{R}^2
\setminus D, D:= D_1\cup \ldots \cup D_n$. Moreover, the distance from
the helicopter to every obstacle should constantly exceed the given
safety margin $d_{\text{safe}}$.
\par
To accomplish this mission, the helicopter has access to the angle
$\beta$ from its forward centerline ray to the target. The sensor
system also scans the region within the sensor range $L$ by rotating
the ray-of-sight and giving the distance $\rho$ to the nearest
obstacle in the current sight direction (if $\rho\leq L$). We assume
that this rotation is fast enough as compared with the robot motion
and neglect effects caused by conventional time sampling of
observations. Modulo this, the helicopter has access to the visible
facet of the obstacle part lying within the sensor range.  So it can
compute the current distance $d(t)$ to the nearest obstacle provided
that $d(t) \leq L$ (otherwise, $d(t):= \infty$). Here
$$
d(t) := \min_{\bldr_\ast \in D} \|\bldr_\ast - \bldr(t)\|, \quad
\|\col(x,y)\| := \sqrt{x^2+y^2}
$$
and $\bldr(t) = \col[x(t),y(t)]$ is the vector of the vehicle
Cartesian coordinates in the world frame.
\clearpage \section{The first method of obstacle avoidance: a sliding mode
  navigation approach}
\label{dbf:bf}
In this section, we assume that the helicopter travels with a constant
speed $v$ and is controlled by the angular velocity $u$ limited by a
given upper bound $u_{\max}$.  The controller design is based on the
following standard unicycle kinematic model:
\begin{equation}
  \dot{x} = v \cos \theta , \quad \dot{y} = v \sin \theta,  \quad
  \dot{\theta} = u, \quad |u| \leq u_{max}, \label{dbf:unicycle}
\end{equation}
where $\theta$ gives the orientation of the helicopter's velocity in
the world frame. The minimal turning radius of the helicopter is thus
given by
\begin{equation}
  \label{dbf:Rmin} R= v/u_{\max}.
\end{equation}
This model is widely used to describe motions of wheeled robots, UAVs,
and missiles; see e.g. \cite{Manchester2004journ9,
  Manchester2006journ2, Kozlowski2009book0}. It also provides a good
modeling framework for a helicopter traveling at a constant speed by
capturing the crucial effect of limitations on the path curvature.
\par
A sliding mode based method for guidance of a unicycle-like vehicle
towards a steady target through the obstacle-free part of the plane
was proposed in \cite{Matveev2011journ2}. This method combines
straight moves to the target with obstacle avoidance maneuvers, with
the former being implemented far enough from the obstacles. Avoidance
maneuvers are arranged by means of a reactive sliding mode navigation
approach, which drives the helicopter to the pre-specified
'comfortable' distance $d_{tar} > d_{safe}$ to the obstacle and then
maintains it.  When in doing so, the helicopter detects the target in
the heading direction, the bypass of the obstacle is terminated and a
straight move to the target is commenced.  As was shown in
\cite{Matveev2011journ2}, this navigation approach ensures achievement
of the control objective under certain technical assumptions.
\par
The navigation approach proposed in \cite{Matveev2011journ2} employs
only the current distance $d(t)$ to the obstacles. Hence it has not
enough data to reasonably judge which side of the encountered obstacle
is favorable for the bypass maneuver.  In this section, we propose a
more informed decision on the choice of this side, which proceeds from
the fact that extended data is available.
\par
Specifically, the following navigation approach is proposed:
\begin{equation}\label{dbf:bfc}
  u(t) = u_{max} \left \{  \begin{array}[ht]{cc}0 & \mid A \\ \Gamma(t) sgn\big\{\dot{d}(t) + X[d(t)-d_{tar} ]\big\} & \mid B \\ \end{array} \right.
\end{equation}

\begin{tabular}{l c p{7cm}}
  $A \rightarrow B$ &:& when $d(t)$ reduces to $d_{trig}$ \\
  $B \rightarrow A$ &:& when the helicopter is oriented towards the
  target (i.e., $\beta(t)=0$) and $d(t) \leq d_{tar} + \epsilon$
\end{tabular}
\vskip0.4\baselineskip
\noindent
Here $sgn$ and $X$ stand for the signum function and the linear
function with saturation, respectively:
\begin{equation}
  \label{dbf:chi}
  X(r) = \left \{  \begin{array}[ht]{cc} lr & |r| < k\\ lk\ sgn(r) & \text{otherwise}
    \end{array} \right. ,
\end{equation}
$d_{tar}, d_{trig},\epsilon >0, l$, $k>0$ are tunable parameters such
that $d_{safe}< d_{tar} < d_{trig} <L$, and $\Gamma(t)$ is generated
by the rule:
\begin{equation}
  \label{dbf:eq.gamma}
  \Gamma (t) :=
  \left\{
    \begin{array}{l l}
      \text{\hspace{-10.0pt}}
      \left.
        \begin{array}{l l}
          -1 &  \text{\hspace{-5.0pt}if}\, |\phi_{l}(t)| \leq |\phi_{r}(t)|
          \\
          +1 & \text{\hspace{-5.0pt}if}\, |\phi_{l}(t)| > |\phi_{r}(t)|
        \end{array}
      \right\}
      & \text{\hspace{-5.0pt} \&} \hspace{5.0pt} d_{trig} \leq d(t) < \infty
      \\
      \Gamma(t^-) & \text{otherwise}
    \end{array}
  \right.
\end{equation}
Writing $\Gamma (t) := \Gamma (t^-)$ means that $\Gamma(\cdot)$ holds
its value; $\Gamma(0)=\pm 1$ is arbitrarily assigned, $\phi_l$ and
$\phi_r$ are the helicopter's angles of sights of the angularly
uppermost and lowermost edges of the visible part of the obstacle,
respectively (see Fig. \ref{dbf:fig:bf}).
\begin{figure}[ht]
  \centering
  \includegraphics[width=.5\columnwidth]{deterministicbf/diagrambf.pdf}
  \caption{The case where motion towards the angularly nearest
    obstacle edge results in a shorter path.}
  \label{dbf:fig:bf}
\end{figure}
\begin{Remark} {\bf (i)} More precisely, $\phi_l, \phi_r \in [-\pi,
  \pi]$ are the polar angles of the edges in the normally oriented
  coordinate frame centered at the vehicle, with the abscissa axis
  directed along its forward centerline ray.
  \par
  {\bf (ii)} Formally, $\phi_l$ and $\phi_r$ are the minimum and
  maximum, respectively, of the angles such that the helicopter
  detects the obstacle in the related direction.
  \par
  {\bf (iii)} The value of $\Gamma(t)$ is of interest only when the
  second line in Eq.\eqref{dbf:bfc} is activated, i.e., when $d(t) \leq
  d_{trig}$. So in fact, employed is the value that is set up at the
  time instant when the helicopter comes to an obstacle at the
  distance $d(t) = d_{trig}$.  Then only one obstacle is visible
  provided that they are distributed sparsely enough: the minimal
  distance between them exceeds the sensor range $L$ plus
  $d_{trig}$. If necessary, this range can be artificially reduced by
  ignoring the distance observations exceeding the desirable range
  $L_{des}$.
  \par
  {\bf (iv)} The navigation approach proposed in
  \cite{Matveev2011journ2} is given by Eq.\eqref{dbf:bfc} with constant
  $\Gamma(t)$. Conversely, the proposed navigation approach makes an
  individual choice of $\Gamma$ for every obstacle avoidance
  maneuver\footnote{Formally, this maneuver is defined as the motion
    during a time interval where the second line from Eq.\eqref{dbf:bfc} is
    constantly activated. Obstacle avoidance maneuvers are
    interspersed by straight moves to the target.}. Informally,
  $\Gamma$ determines whether the obstacle is transversed in a
  clockwise or counter-clockwise direction.
  % \par
  % {\bf (v)} By Eq.\eqref{dbf:bfc}, an obstacle avoidance maneuver basically
  % commences with $\dot{d}<0$. Moreover, both the requirements to the
  % controller parameters $l$ and $k$ in Eq.\eqref{dbf:chi} and the arguments
  % from the proofs presented in \cite{matveev_method_2010} entail
  % that typically $\dot{d}< - lk$. Then $sgn \{\ldots \} =-1$ in the
  % second line from Eq.\eqref{dbf:bfc} and so the avoidance maneuver starts
  % with an abrupt turn (with $|u|=u_{\max}$), which is clockwise if
  % $\Gamma =1$ and counter-clockwise if $\Gamma=-1$. This direction
  % is fixed for the law from \cite{matveev_method_2010}, whereas the
  % proposed law chooses it individually for every avoidance maneuver
  % with regard to the situation at its start.
  \par
  {\bf (vi)} The direction is chosen towards the obstacle edge that
  has the smallest angular difference with the target direction (in
  which the helicopter moved just before the start of the avoidance
  maneuver due to Eq.\eqref{dbf:bfc}). This seems to be a reasonable choice
  for estimating which direction would result in a shorter path
  {\color{blue}(see figure \ref{dbf:fig:bf})}\footnote{Of course,
    there are situations where the chosen direction is in fact
    worse. However, it is reasonable to assume that decision based on
    what is currently visible cannot be worse on average than a
    completely uninformed decision.}.
\end{Remark}
\par
To state the convergence properties of the proposed navigation
approach, we need some assumptions, mostly borrowed from
\cite{Matveev2011journ2}.
\begin{enumerate}[{\bf $\mathcal{A}$.1)}]
\item \label{dbf:ass.a1} \textit{Obstacle shape:} any obstacle $D_i$
  is compact and convex; its boundary is piecewise smooth.
\item \textit{Obstacle spacing:} The obstacles are disjoint and
  separated by the large enough distance:
  \begin{multline*}
    \text{\bf dist}\; [D_i, D_j] := \inf_{\boldsymbol{r}^\prime \in
      D_i, \boldsymbol{r}^\pprime \in D_j}\| \boldsymbol{r}^\prime -
    \boldsymbol{r}^\pprime\|
    \\
    > 2 \left( 3R+ \max \big\{ d_{safe}; R \big\}\right) \qquad i \neq
    j .
  \end{multline*}
  Here $R$ is the minimal turning radius Eq.\eqref{dbf:Rmin} of the
  helicopter.
\item \textit{Range measurement:} The helicopter measures the distance
  $d_i(t)$ to the obstacle $D_i$ whenever $d_i(t) \leq L$, where the
  visibility range $L$ is large enough:{
    \begin{equation}
      \label{dbf:ld} L> 4R+\max\{R; d_{safe}\}.
    \end{equation}
    This inequality is inspired by the fact that according to
    Eq.\eqref{dbf:bfc}, the helicopter starts the bypass maneuver when the
    distance $d$ to the obstacle decreases to $d_{trig}$ and then
    moves over a circle with the radius $R$ until the expression in
    the curly brackets from Eq.\eqref{dbf:bfc} vanishes. In doing so, it may
    reach a distance $d \in \Delta :=\left[ d_{trig} - 2R, d_{trig} +
      2R \right]$. It is natural to demand that $d_{trig} - 2R \geq
    d_{safe}$ because of the safety concerns and that for all $d \in
    \Delta$, the helicopter should not lose control over the distance
    to the obstacle, i.e., be able to both increase and decrease
    it. This means that the minimal turning radius $R$ of the vehicle
    should be less than $d$ plus the curvature radius of the obstacle
    boundary. Since no lower bounds are imposed on the latter radius,
    we get $d \geq R$ and overall, $d_{trig} - 2R \geq \max\{
    d_{safe}, R \}$. On the other hand, implementation of Eq.\eqref{dbf:bfc}
    requires that the sight of the obstacle must be maintained during
    the entire bypass maneuver $L > d_{trig} + 2R$. By excluding the
    controller parameter $d_{trig}$, we arrive at Eq.\eqref{dbf:ld}.  }
\item \label{dbf:ass.alast} \textit{Target location:} The target is
  far enough from the obstacles: the distance from $T$ to $D$ exceeds
  $\max \{d_{safe}; R\}$.
\end{enumerate}
\par
To ensure convergence, a special choice of the parameters $d_{tar},
\epsilon, d_{trig}, l$, and $k$ is recommended in
\cite{Matveev2011journ2}. To describe it, we denote by
$R_{\varkappa}(r|\partial D_i)$ the curvature radius of the boundary
$\partial D_i$ at the point $r \in \partial D_i$ (for the corner
points, $R_{\varkappa}(r|\partial D_i):= 0$) and consider the minimum
among them:
$$
R_- := \min_{i=1,\ldots,n} \inf_{r \in \partial D_i}
R_{\varkappa}(r|\partial D_i).
$$
The parameters should be chosen so that {\color{blue}
  \begin{gather}
    \nonumber d_{tar} > \max\big\{d_{safe}; R-R_- \big\}; \qquad
    \epsilon >0 ;
    \\
    \nonumber \max\big\{ d_{tar}+\epsilon; d_{safe}+2R; 3R \big\} <
    d_{trig}
    \\
    \nonumber < \min \left\{ L -2R ; \frac{1}{2} \min_{i \neq j}
      \text{\bf dist}\; [D_i, D_j] -R \right\};
    \\
    \label{dbf:main.cond1} \sqrt{1+\frac{l^2}{(1-\frac{R}{\text{min}\{
          d_{tar}, d_{trig} - 2R\}+R_-})^2 u_{\max}^2}} < \frac{v}{l
      k} .
  \end{gather}
} Under assumptions
$\mathcal{A}$.\ref{dbf:ass.a1})---$\mathcal{A}$.\ref{dbf:ass.alast}),
such a choice is possible \cite{Matveev2011journ2}. To establish the
convergence, we impose one more requirement $\mathcal{A}$.5), which
concerns both the distribution of the obstacles over the plane and the
choice of the controller parameters. To state it, we introduce the
following.
\begin{Definition}
  \label{dbf:neigh}
  For $c \in (0,+\infty)$, the $c$-neighborhood $\mathcal{N}[c,D]$ of
  the set $D$ is defined as follows:
  \begin{equation}
    \mathcal{N}[c,D] := \{z \in \mathbb{R}^2 :\min\limits_{\acute{z} \in D}\|z - \acute{z}\| \leq c \}.
  \end{equation}
\end{Definition}
\begin{enumerate}
\item[{\bf $\mathcal{A}$.5)}] \textit{Non-blocking:} For any pair of
  obstacles $D_i, D_j, i \neq j$ such that the line segment extending
  from some point on $\partial\mathcal{N}[d_{tar} + \epsilon,D_i]$ to
  the target $T$ intersects $\mathcal{N}[d_{trig},D_j]$, the
  inequality $\|z_i - T\| > \|z_j - T\|$ holds for any points $z_i
  \in \partial \mathcal{N}[d_{tar} + \epsilon, D_i], z_j \in \partial
  \mathcal{N}[d_{tar} + \epsilon, D_j]$.
\end{enumerate}
Recall that by Eq.\eqref{dbf:bfc}, $d_{tar}+\epsilon$ is the distance to
$D_i$ within which the helicopter may be switched from bypassing the
obstacle $D_i$ to the straight move to the target. Furthermore,
$d_{trig}$ is the distance to $D_j$ at which the straight move to the
target is replaced by bypassing the obstacle $D_j$.  So with a slight
abuse of exactness, $\mathcal{A}$.5) means that any obstacle $D_j$
capable to obstruct the straight move to the target after bypassing
$D_i$ lies, as the whole, closer to the target than $D_i$.
\par
The following theorem is the main result of the section.
\begin{Theorem}
  \label{dbf:T2} Let assumptions~{\rm
    $\mathcal{A}$.\ref{dbf:ass.a1})---$\mathcal{A}$.5)} and
  inequalities Eq.\eqref{dbf:main.cond1} hold. There exists $\epsilon_*>0$
  such that for any $0<\epsilon<\epsilon_*$, the navigation law
  Eq.\eqref{dbf:bfc}---Eq.\eqref{dbf:eq.gamma} drives the helicopter to the target
  for a finite time $\exists t_f>0: \boldsymbol{r}(t_f)
  =\boldsymbol{T}$ and ensures the safety requirement $d(t)\geq
  d_{safe} \; \forall t\in [0,t_f]$ provided that initially the
  vehicle is not at the target $\boldsymbol{r}(0)\neq T$, moves
  towards it $\beta(0)=0$, and is far enough from the obstacles $d(0)
  \geq d_{trig}$.
  % outside the set ${\cal N}[d_{trig},D]$.
\end{Theorem}
\pf In fact, this theorem was established in \cite{Matveev2011journ2}
for the case where the machinery Eq.\eqref{dbf:eq.gamma} is switched off and
$\Gamma(t)\equiv \pm 1$ is kept constant. At the same time,
$\Gamma(t)$ influences the navigation approach output only during
obstacle avoidance maneuvers; and during bypass of any particular
obstacle, the proposed machinery Eq.\eqref{dbf:eq.gamma} keeps $\Gamma(t)$
constant. It follows that it does not affect the arguments from the
proof of Theorem~5.1 in \cite{Matveev2011journ2}, and the proof of the
current theorem is achieved by mere retracing them. \epf

{
  \subsection{Preliminary Comparison to Model Predictive Control}
  Our simultaneous interest to two control methods
  % (sliding-mode and model predictive control, respectively)
  is partly motivated by the fact that they provide complementary
  benefits. The controller from Sec.~\ref{dbf:bf} consumes extremely
  low computational power and demands mild sensing
  capabilities. However if this power and capabilities are not
  strongly limited, this means refrainment from utilizing the full
  strengths of the computing and sensing modules, which carries a
  potential of performance degradation as compared with more informed
  and implementable control strategies. This partly concerns the
  situation at hand, where the vehicle has access not only to the data
  consumed by the controller from Sec.~\ref{dbf:bf} but also to the
  entire local part of the scene within the given sensor range. Then
  model predictive control (MPC) approach seems to be capable of
  ensuring better performance so far as it involves on-line
  optimization subject to constraints that may be dynamically adjusted
  to the constantly changing current knowledge about the
  environment. However MPC is partly based on heuristics and does not
  ensure strict optimality \cite{MaRaRaSc00}.
  \par
  Typically, theoretical analysis of the overall optimality features
  of MP controllers is a hard task \cite{MaRaRaSc00}, with the result
  being not unambiguous. In view of this, we limit ourselves to merely
  a theoretical illustration aimed to compare, in a refined and
  simplified setting, the principles embodied by the proposed two
  control laws. Extended experimental comparison of the laws
  themselves will be offered in Sects.~\ref{dbf:sim} and
  \ref{dbf:exp}.
  \par
  To establish a compromise between the models, now the helicopter is modeled
  as a point moving with the constant speed $v$ and controlled by the
  velocity orientation.  This model is nearly equal to
  Eq.\eqref{dbf:unicycle} with $u_{\max} := \infty$, which allows for
  arbitrarily sharp turns. We examine bypass of a prolonged
  rectangular obstacle with negligible thickness, which can thus be
  modeled as a long segment of a straight line. At the start of the
  maneuver, the vehicle's move to the target in a straight line is
  obstructed by the obstacle; see Fig.~\ref{dbf:fig.comp}.
  \begin{figure}[ht]
    \centerline{
      \scalebox{0.5}{\includegraphics{deterministicbf/comp.pdf}}}
    \caption{Bypass of a straight obstacle according to two principles
      of control.} \label{dbf:fig.comp}
  \end{figure}
  The control law from Sec.~\ref{dbf:bf} implements, by means of the
  sliding-mode technique, the principle: move to the target in a
  straight line whenever this is possible, and follow the obstacle
  boundary otherwise. Under the circumstances, this results in the
  route $A \mapsto B \mapsto C \mapsto D \mapsto T$. To compare with,
  we consider the MP control principle: apply the control that is
  optimal for the currently visible scene, with the performance index
  being the length of the path. This means that the vehicle first
  moves to the target in a straight line until this move is not
  obstructed by the visible part of the obstacle. At point $B$ where
  the distance to the edge of this part increases up to the visibility
  range $L$, the vehicle starts moving so that it is constantly headed
  to this edge. This motion is curvilinear before point $E$ where this
  edge arrives at the real edge of the obstacle, and linear after this
  point. Thus the vehicle follows the route $A \mapsto B \mapsto E
  \mapsto D \mapsto T$. In the compared two paths, the parts $A
  \mapsto B$ and $D \mapsto T$ are common, whereas $B \mapsto C$ and
  $E \mapsto D$ have the common length $L$. Thus we in fact have to
  compare the lengths of the linear $C \mapsto D$ and non-linear $B
  \mapsto E$ paths. In the following lemma, we examine the maneuver
  that starts before point $B$ and assume that at this point, the edge
  of the visible part of the obstacle is not the real edge and that
  both paths involve the right turn to bypass the obstacle.
  \begin{Lemma}
    \label{dbf:lem.comp} The performance of the first control law
    (evaluated by the length of the path $A \mapsto B \mapsto C
    \mapsto D \mapsto T$) is always worse than that of the MP law. The
    over-performance (evaluated by the difference between the lengths
    of the paths $A \mapsto B \mapsto C \mapsto D \mapsto T$ and $A
    \mapsto B \mapsto E \mapsto D \mapsto T$) does not exceed $L \ln
    2$ and approaches this bound as the obstacle extends to the right
    without limits and the angle $\alpha$ from Fig.~{\rm
      \ref{dbf:fig.comp}} takes the value $\frac{\pi}{2}$.
  \end{Lemma}
  \par
  \pf At any point of the path $B \mapsto E$, the edge of the visible
  part of the obstacle lies on the tangential line at the distance $L$
  from this point. So in the Cartesian frame introduced in
  Fig.~\ref{dbf:fig.comp}, the coordinates $(x_e,y_e)$ of this edge
  are related to those $(x,y)$ of the vehicle by $x_e = x+
  \sqrt{L^2-y^2}, y_e=0$, and
$$
\left( \begin{array}{c} \dot{x}\\ \dot{y} \end{array}\right) =
\frac{v}{L} \left( \begin{array}{c} x_e-x\\ y_e-y
  \end{array}\right) =
\frac{v}{L} \left( \begin{array}{c} \sqrt{L^2-y^2} \\ - y
  \end{array}\right).
$$
Denoting by $s$ the length of the path passed along $B \mapsto E$, we
have
\begin{multline*}
  \dot{s} =v, \quad \frac{d y}{ds} = - \frac{y}{L}, \quad y(s) =
  y_0e^{- \frac{s}{L}},
  \\
  \dot{x}_e = \dot{x} - \frac{y \dot{y}}{\sqrt{L^2-y^2}} = \frac{v}{L}
  \left[ \sqrt{L^2-y^2} + \frac{y^2}{\sqrt{L^2-y^2}}\right] =
  \frac{vL}{\sqrt{L^2-y^2}} = \frac{L}{\sqrt{L^2-y^2}} \dot{s} .
\end{multline*}
Now we observe that as the vehicle performs the move $B \mapsto E$,
the point $x_e$ runs over $C \mapsto D$. Hence by denoting
$S:=\mathscr{L} [C \mapsto D]$, where $\mathscr{L}$ stands for the
length of the path, we see that
$$
\Delta:=\mathscr{L} [C \mapsto D] - \mathscr{L} [B \mapsto E] =
\int_0^S \left[ \frac{1}{\sqrt{1-\frac{y^2}{L^2}}} -1 \right] \; ds
>0.
$$
Thus the first claim of the lemma is true.
\par
Given the conditions at point $B$, the difference $\Delta$ increases
as the obstacle extends to the right, and for very long obstacles,
approaches the limit value
$$
\Delta \to \int_0^\infty \left[ \frac{1}{\sqrt{1- L^{-2} y_0^2
      e^{-2s/L}}} -1 \right] \; ds \overset{\zeta=
  L^{-1}|y_0|\exp(-s/L)}{=\!=\!=\!=\!=\!=\!=\!=\!=\!=\!=} L
\int_0^{\frac{|y_0|}{L}} \left[ \frac{1}{\sqrt{1- \zeta^2}} -1 \right]
\frac{1}{\zeta} \; d \zeta
$$
Given the visibility range $L$, the expression on the right attains
its maximum at $|y_0| = L$ (i.e., for $\alpha = \pi/2$). This maximum
is equal to
\begin{multline*}
  L \int_0^{1} \left[ \frac{1}{\sqrt{1- \zeta^2}} -1 \right]
  \frac{1}{\zeta} \; d \zeta \overset{\zeta = \sin \tau}{=\!=\!=\!=} L
  \int_0^{\frac{\pi}{2}} \left[ \frac{1}{\cos \tau} -1\right]
  \frac{\cos \tau}{ \sin \tau} \; d\tau = L \int_0^{\frac{\pi}{2}}
  \tan \frac{\tau}{2}\; d \tau
  \\
  = - 2 L\ln \cos \frac{\tau}{2} \Big|_{\tau=0}^{\tau = \frac{\pi}{2}}
  = - 2 L \ln \frac{\sqrt{2}}{2} = L \ln 2,
\end{multline*} \epf
\par
By Lemma~\ref{dbf:lem.comp}, MPC law over-performs the sliding mode
one.  The over-performance may be arbitrarily large provided that the
visibility range is large enough, though it is upper bounded for a
given range. It should be stressed that these claims are based on
simplifying assumptions. The next section offers more detailed and
reliable comparative analysis of two proposed control laws.}



\clearpage \section{Simulations}
\label{dbf:sim}

For the sliding mode control, the desired heading was actuated, while
keeping the speed constant.

\begin{table}[ht]
  \centering
  \begin{tabular}{| l | c |}
    \hline
    $u_{max}$ & $1.3 rads^{-1}$ \\
    \hline
    $v$ & $1.5 ms^{-1}$ \\
    \hline
    $R$ & $2 m$  \\
    \hline
    $d_{tar}$ & $5 m$  \\
    \hline
    $d_{trig}$ & $10 m$ \\
    \hline
    $l$ & $0.33$  \\
    \hline
    $k$ & $15m$  \\
    \hline
  \end{tabular}
  \caption{Parameters used for simulations}
  \label{dbf:dbf:param}
\end{table}

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.5\columnwidth]{deterministicbf/lfbf.pdf}
  \caption{Results obtained from the boundary following algorithm,
    using the unicycle model.}
  \label{dbf:fig:lfbf}
\end{figure}



\begin{figure}[ht]
  \centering
  \includegraphics[width=0.5\columnwidth]{deterministicbf/hfbf.pdf}
  \caption{Results obtained from the boundary following algorithm,
    using the realistic helicopter model.}
  \label{dbf:fig:hfbf}
\end{figure}






For all these simulations, the controller refresh rate of 5 Hz was
used. The parameters used for control can be found in table
\ref{dbf:dbf:param}.  For all navigation approaches and vehicle
models, the obtained trajectories appear to be similar, being able to
guide the helicopter without collision. The model predictive approach
achieves significantly faster velocities than the boundary following
approach (as is expected). The boundary following navigation is most
limited in that it assumes the turning radius is under a threshold
compared to the obstacle separation, and the helicopter must travel at
a low speed to ensure this. However it has the advantage of
simplicity, and would require significantly less computation resources
than the model predictive approach.


\begin{Remark}
  The model predictive controller is less restrictive as it does not
  impose constraints on the environment, whereas the sliding mode
  navigation approach relies on assumptions about the obstacle
  curvature. To satisfy them, the helicopter has to adopt its cruise
  speed to any potential obstacle. For the scene with highly contorted
  obstacles, this may mean that the helicopter has to travel very
  slowly, which may be undesirable.
\end{Remark}


\clearpage \section{Experimental results with a wheeled robot}
\label{dbf:exp}
Both navigation approaches were also tested on the Pioneer P3-DX
mobile robot, to show their viability on a real world hardware
platform. Performing real world tests with helicopters requires many
more resources and risk. For the sliding mode controller, the control
signal was applied directly as the robot's desired rotation rate. In
order to interface the robot with control obtained from the local path
planning, the desired speed was set to be $\|v^*(1|k)\|$, and the
desired rotation rate set to be proportional to the angle between the
vehicle and the first waypoint, $\dot{\theta} := k \cdot
[\text{angle}(s^*(1|k) - s(k)) - \theta(k)]$, which tends to navigate
the vehicle towards this point \cite{Aicardi1995journ4}. While a
wheeled robot technically has non-holonomic constraints, the model
predictive algorithm can still cope with this and guide the robot
satisfactorily.

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.5\columnwidth]{mobilesimbw.png}
%   \caption{Simulations obtained by interfacing the model
%   predictive navigation approach {\color{blue}with the wheeled robot
%   control
%   software \cite{pioneer}}. {\color{blue} The target
%   point is sufficiently far away, so the control goal is nearly
%   equivalent
%   to tracking a certain heading.}}
%   \label{dbf:fig:mobilesim}
% \end{figure}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.5\columnwidth]{mobilesimbfbw.png}
%   \caption{The same simulation as in {\color{blue} figure
%   \ref{dbf:fig:mobilesim}}, using the boundary following navigation
%   approach.}
%   \label{dbf:fig:mobilesimbf}
% \end{figure}

\begin{figure}[ht]
  \begin{tabular}{cc}
    \includegraphics[width=0.35\columnwidth]{s1bw.jpg} & \includegraphics[width=0.35\columnwidth]{s2bw.jpg}\\
    \includegraphics[width=0.35\columnwidth]{s3bw.jpg} & \includegraphics[width=0.35\columnwidth]{s4bw.jpg}\\
    \includegraphics[width=0.35\columnwidth]{s5bw.jpg} & \includegraphics[width=0.35\columnwidth]{s6bw.jpg}\\
  \end{tabular}\\
  \caption{Sequence of images showing the model predictive navigation
    approach in action}
  \label{dbf:pics}
\end{figure}

 The
  maneuver for the model predictive approach took approximately 22
  seconds, while the same maneuver for the sliding mode approach took
  approximately 52 seconds, which again indicates that the model
  predictive control algorithm is superior.

A limitation on this platform is that the laser rangefinder is forward
facing, which limits the path planning and has the potential to stop
the robot at certain local minima {\color{blue}, such as in the final
  image in figure \ref{dbf:pics}}. A simple heuristic fix would be to
instruct the robot to rotate if it is stationary and no paths can be
planned.

\clearpage \section{Summary}
\label{dbf:conc}
Two robust approaches to navigate a helicopter to a target while
bypassing en-route obstacles are presented. The approach based on the
model predictive control was found to be superior and be able to avoid
obstacles under all circumstances. The other algorithm employs sliding
mode navigation and is partly aimed at maintaining the given distance
to the obstacle boundary. Whereas this algorithm is mathematically
simpler, the necessary assumptions make it unsuitable for high
speeds. Applications of this concept could include navigation of
helicopters in confined areas, where utmost consideration must be
given to safety. Future work on this subject will look at extending it
to cooperative scenarios, as well as performing real world tests on
autonomous helicopters.

